A Domain-Independent Agent Architecture for Adaptive Operation in Evolving Open Worlds

Model-based reasoning agents are ill-equipped to act in novel situations in which their model of the environment no longer sufficiently represents the world. We propose HYDRA - a framework for designing model-based agents operating in mixed discrete-continuous worlds, that can autonomously detect when the environment has evolved from its canonical setup, understand how it has evolved, and adapt the agents' models to perform effectively. HYDRA is based upon PDDL+, a rich modeling language for planning in mixed, discrete-continuous environments. It augments the planning module with visual reasoning, task selection, and action execution modules for closed-loop interaction with complex environments. HYDRA implements a novel meta-reasoning process that enables the agent to monitor its own behavior from a variety of aspects. The process employs a diverse set of computational methods to maintain expectations about the agent's own behavior in an environment. Divergences from those expectations are useful in detecting when the environment has evolved and identifying opportunities to adapt the underlying models. HYDRA builds upon ideas from diagnosis and repair and uses a heuristics-guided search over model changes such that they become competent in novel conditions. The HYDRA framework has been used to implement novelty-aware agents for three diverse domains - CartPole++ (a higher dimension variant of a classic control problem), Science Birds (an IJCAI competition problem), and PogoStick (a specific problem domain in Minecraft). We report empirical observations from these domains to demonstrate the efficacy of various components in the novelty meta-reasoning process.

==> evaluation.tex <==
HYDRA has been implemented and evaluated for three domains: CartPole++, ScienceBirds, and PogoStick. 

%\subsection{Case Study Domains}

%\roni{Pasting here the text about the domains from above. Should be editted to avoid repeating what's said in section 3}
%\subsection{Science Birds}

%The video game Science Birds has garnered widespread recognition over a substantial number of years. Its objective involves eliminating all green pigs in a level while maximizing destruction to the surrounding structures. The player is equipped with a collection of birds, which may vary, to be launched from a slingshot. The pigs are typically concealed within complex structures, requiring the player to identify and eliminate the weak points of the structures, such as supports or dynamite. The development of Science Birds utilized the Box2D open-source physics library, ensuring that all objects within the game's environment comply with the principles of Newtonian physics in a two-dimensional plane.
%An example of a novelty in this domain is to change how gravity affects the yellow birds. 

% In this context, the Science Birds game used is a modified-dimensional version of the standard Science Birds benchmark, incorporating various novelties. The novelties of Science Birds are divided into three phases based on their order of release date. Each phase of novelties contains different levels and types corresponding to the difficulties posed by the induced novelties in the game. 
% A detailed description of each novelty is presented in Table ~\ref{tab:sb_novelties}.
% %%%%%%%%%%%%%%%%%%
% %https://gitlab.com/aibirds/sciencebirdsframework/-/blob/release/alpha0.6.3/novelty_descriptions.md
% \begin{table}[h!]
% \begin{tabular}{|llp{0.8\linewidth}|}
% \Xhline{2\arrayrulewidth}
% \Xhline{1.5pt}  
% %\hline
% \multicolumn{3}{|c|}{\textbf{Phase 1}}    %\\ \hline
% \\\Xhline{2\arrayrulewidth}
% \Xhline{1.5pt}  
% \multicolumn{1}{|l|}{\textbf{Level}} & \multicolumn{1}{l|}{\textbf{Type}} & \textbf{Description}                       \\ \hline
% \multicolumn{1}{|l|}{11}             & \multicolumn{1}{l|}{50}            & Styroform Black \roni{What is this? a new type of block?} (wood health x 4, mass reduce 90\%)                                                                    \\ \hline
% \multicolumn{1}{|l|}{11}             & \multicolumn{1}{l|}{130}           & No wood damage for orange bird                                                  \\ \hline
% \multicolumn{1}{|l|}{12}             & \multicolumn{1}{l|}{30}            & Yellow bird launch gravity increase to 0.7                                                                             \\ \hline
% \multicolumn{1}{|l|}{12}             & \multicolumn{1}{l|}{110}           & Blue Bird Split to 5                                                                                                   \\ \hline
% \multicolumn{1}{|l|}{13}             & \multicolumn{1}{l|}{20}            & Remove blue channel of the colours of objects                                                      \\ \hline
% \multicolumn{1}{|l|}{13}             & \multicolumn{1}{l|}{90}            & Shift the coordinate origin to the center point of the slingshot                                         % \\ \hline
% \\\Xhline{2\arrayrulewidth}
% \Xhline{1.5pt}  
% \multicolumn{3}{|c|}{\textbf{Phase 2}}                                                         
% \\\Xhline{2\arrayrulewidth}
% \Xhline{1.5pt}  
% \multicolumn{1}{|l|}{22}             & \multicolumn{1}{l|}{40-44}         & Bird Teleporters send a contacted objectto the other gate                                              \\ \hline
% \multicolumn{1}{|l|}{22}             & \multicolumn{1}{l|}{50-54}         & A space invader that moving horizontally and hits the directly reachable objects underneath with a laser beam          \\ \hline
% \multicolumn{1}{|l|}{23}             & \multicolumn{1}{l|}{40}            & The witch is a bird chaser now that actively speeds up and attempts to hit any birds that is within a certain distance \\ \hline
% \multicolumn{1}{|l|}{23}             & \multicolumn{1}{l|}{70}            & The witch is an immortalizing agent that makes all the pigs immortal if it is killed                                   \\ \hline
% \multicolumn{1}{|l|}{24}             & \multicolumn{1}{l|}{60-64}         & The TNT is now a bird nest that will provide two more red birds if it is destroyed                                     \\ \hline
% \multicolumn{1}{|l|}{24}             & \multicolumn{1}{l|}{70-74}         & The red bird can go through platforms                                                                                  \\ \hline
% \multicolumn{1}{|l|}{25}             & \multicolumn{1}{l|}{60-63}         & The platforms will move up and down                                                                                    \\ \hline
% \multicolumn{1}{|l|}{25}             & \multicolumn{1}{l|}{70-74}         & The TNT power cannot go through the platforms anymore                                                        %          \\ \hline
% \\\Xhline{2\arrayrulewidth}
% \Xhline{1.5pt} 
% \multicolumn{3}{|c|}{\textbf{Phase 3}}                                                                                                                                                 \\\Xhline{2\arrayrulewidth}
% \Xhline{1.5pt} 

% \multicolumn{1}{|l|}{36}             & \multicolumn{1}{l|}{10-14}         & No gravity for birds                                                                                                   \\ \hline
% \multicolumn{1}{|l|}{36}             & \multicolumn{1}{l|}{20-24}         & A radioactive area that will kill any bird that touches it                                                             \\ \hline
% \multicolumn{1}{|l|}{37}             & \multicolumn{1}{l|}{10}            & The magician acts as a transmuter who turns any touched object to a pig                                                \\ \hline
% \multicolumn{1}{|l|}{37}             & \multicolumn{1}{l|}{20}            & The butterfly adds health points to the pigs nearby                                                                    \\ \hline
% \multicolumn{1}{|l|}{38}             & \multicolumn{1}{l|}{10-14}         & A time triggered storm that applies force to the left of the flying birds                                              \\ \hline
% \multicolumn{1}{|l|}{38}             & \multicolumn{1}{l|}{20-24}         & A long wood object will destroy itself when a bird collides with any object                                       \\ \hline
% \end{tabular}
% \caption{Description of novelties in each level and type released by three phases \roni{These numbers of types and levels are just internal IDs, no? if so, we should just omit them.}}
% \label{tab:sb_novelties}
% \end{table}
% %%%%%%%%%%%%%

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.85\columnwidth]{images/cartpole.png}
 %/   \caption{Screenshot of CartPole++ environment.}
%/    \label{fig:cartpole}
%\end{figure}

%\subsection{Cartpole++}
%Cartpole++ is a physics-based discrete-continuous domain. The CartPole++ environment (seen in figure \ref{fig:cartpole}) is a higher-dimensional version of the standard Reinforcement Learning benchmark, with more actions and state variables. The planning agent rely solely on PDDL+ model of the CartPole++ environment to solve the non-novel instances. For each episode, the agent generates a problem file from the initial environment observation (i.e., initial positions and velocities of the cart and pole) and default assumptions about the environment (i.e., gravity, masses of cart and pole, etc.). The expressiveness of PDDL+ enabled us to holistically encode the CartPole++ system dynamics as a planning domain (without using any external functions/solvers). Despite inherent complexity, efficient modeling allowed the use of off-the-shelf PDDL+ planners to solve the resulting problems. The planners were required to handle non-linear dynamics, large numbers of active happenings, and long temporal horizons.
%Depending on the initial positions, our planner can solve full 200-step CartPole PDDL+ problems in under $1.0$ second using GBFS algorithm with a domain specific heuristic prioritizing ``safe" states (pole close to the vertical). To account for the inherent noise between the planner and the execution environment, every 10 steps the agent re-plans for the remainder of the episode.  
% We built two versions of the model-based planning agent. \emph{Planning-static} agent uses the same PDDL+ model for both the non-novelty and novelty setup. \emph{Planning-adaptive} agent monitors plan execution and automatically repairs the PDDL+ model inconsistency is detected using \emph{focused model repair}, as proposed in section \ref{sec:agent}. \emph{Repairable fluents} are all parameters defining CartPole dynamics. To estimate the inconsistency score $C$ (from Section \ref{sec:inconsistency}), the adaptive planning agent uses Euclidean distance over only pose of the cartpole (i.e., $\tuple{cart\_x, cart\_y, theta\_x, theta\_y}$). In non-nominal case $C{=}0$, while the threshold was set to $C_{th}{=}0.009$.


%\subsection{PogoStick}
%\textcolor{red}{\emph{Assumption ($\sim$Sachin) -- this talks about how T* changes are handled in Pogostick. As this is the first time PogoStick is talked about, we also need to explain the domain here.}}
%\roni{I think better to explain very briefly the domains above, as I did, and then here only put the specifics used in our experiments}

%\begin{figure}
%\centering
%\includegraphics[width=\textwidth]{images/polycraft_environment.png}
%\caption{Top- and first-person view of the simulated environment for polycraft. Steve interacts with environment by sending sequence of commands such as ``SENSE\_ALL'' or ``BREAK BLOCK'' for cutting trees of mining ores in the environment.}
%\label{fig:polycraft_environment}
%\end{figure}

%PogoStick is a MineCraft\footnote{\url{https://www.minecraft.net/}} based domain (sometimes called PolyCraft), where an agent (Steve) has to construct a pogostick. Steve has to interact with the environment, gather resources such as logs by cutting trees or through mining ores of platinum, diamond, etc., interact with other entities such as traders to trade for several other resources, and follow a recipe to construct a pogostick.
%Steve's task has several challenges as it has to perform sequential decision-making tasks that require both short and long-term planning. For example, it has to decide the resources needed to craft intermediate products, such as, a tree tap, and then use it to collect rubber for curating a pogostick from a specific kind of a tree in the environment. Figure \ref{fig:polycraft_environment} shows the top- and first-person view of the environment that consists of 30x30 grass field, and is connected to two smaller rooms. 

%Steve has the ability to interact with the environment by sending commands to the simulator. For example, steve can sense the environment by sending ``SENSE\_ALL'' command to the simulator and the simulator responds with the entities in the environment, their location, Steve's inventory, etc. Each action executed in the simulator has some cost attached to it (in the order of 1000 points), and Steve is rewarded with 256,000 points for a constructing a pogostick. The final score (reward - cost of executing all the actions) is presented after completion of the episode.

%Although, constructing a pogostick has it's own challenges, diverging $T^*$ due to novelty provides a completely new challenge for the agent. Novelties can support/hinder the construction of the pogostick, such as, by changing the quantity of raw material from their ores, or wind in the environment that changes the location of the agent while moving in the environment. 
%A trial in polycraft environment consists of 50-100 episodes, and the novelty is introduced roughly after $20\%$ of the episodes have been completed. The agent should report the novelty after it has been introduced and update it's own transition function to incorporate the effects of novelty.



\subsection{Novelty Detection}
\subsubsection{Visual Reasoning}
\subsubsection{Reward Estimation}
\subsection{Novelty Accommodation}



\subsection{CartPole}
Our first set of experiments were designed to measure if learning by model repair can accommodate novelties online. We use the standard CartPole implementation provided by the OpenAI Gym\footnote{https://gym.openai.com} for implementation and experiments.  In the CartPole domain, the agent's task is to balance the pole in the upright position for $n=200$ steps by pushing the cart either left or right. The domain's system dynamics are defined by several parameters: mass of the cart, mass of the pole, length of the pole, gravity, angle limit, cart limit, push force. The CartPole environment only provides information on the velocities and positions of the cart and the pole (4-tuple). The agent has two actions, left and right, that apply a constant force. Every step returns a $+1$ reward unless the pole diverges from vertical by $\pm 12^{\circ}$, at which point the episode ends in a loss.

\subsubsection{Experiments} Our first set of experiments is designed to evaluate if the proposed model repair method can enable a planning agent to adapt to novelties in open worlds. Recall that a novelty implies a sudden, unknown, and unexpected change in environment dynamics. We structured our experiments as a set of $t=5$ trials consisting of $l=200$ episodes each. Each trial begins with episodes in nominal conditions. Novelty is introduced after $k=7$ canonical episodes where the environmental parameters are changed without informing the agent. Reward obtained by the agent in each episode is recorded. We report our observations on two novelties: length of the pole is updated to $1.1$, gravity to $12$; and length of the pole to $1.1$ and mass of the cart is decreased to $0.9$. These novelties were selected because they impact the performance of all agents tested significantly. 


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Domain                        & Repairable var.       & Nom. val. & $\Delta$  \\ \midrule
% \multirow{5}{*}{Angry Birds} & bird velocity         & 0.000     & 50.000 \\
%                               & gravity               & 9.810     & 1.000  \\
%                               & wood block multiplier & 1.000     & 1.000  \\
%                               & ice block multiplier  & 1.000     & 1.000  \\
%                               & stoneblock multiplier & 1.000     & 1.000  \\\midrule
\multirow{3}{*}{Angry Birds} & bird velocity change  & 0.000     & 1.000 \\
                              & pig life multiplier   & 0.000     & 50.000  \\
                              & gravity factor        & 9.810     & 0.100  \\\midrule
\multirow{7}{*}{CartPole}     & mass cart             & 1.000     & 1.000  \\
                              & length pole           & 0.500     & 0.100  \\
                              & mass pole             & 0.100     & 0.100  \\
                              & force magnitude       & 10.000    & 1.000  \\
                              & gravity               & 9.810     & 1.000  \\
                              & pole angle limit      & 0.205     & 0.100  \\
                              & cart position limit   & 2.400     & 0.100  \\
                            %   \cmidrule(l){2-4} 
                            \bottomrule
\end{tabular}

\caption{Domain-specific parameters for PDDL+ model repair. Lists for each domain, the repairable state variables, their nominal value, and the $\Delta$ values used when trying to repair. \roni{@Sachin: can you add Polycraft here?}\label{tab:domain-paramaters}}
\end{table}


\subsubsection{Planning Agents}
% \begin{table*}[h]
%     \centering
%     \small
%     \begin{tabular}{l|lcccccccc}
%     \toprule
%         \textbf{repairable fluents} &  \texttt{mass cart}& \texttt{length pole}& \texttt{mass pole}& \texttt{force magnitude}& \texttt{gravity}& \texttt{pole angle limit}& \texttt{cart position limit}\\
%         \textbf{nominal values} &1.0&0.5&0.1&10.0&9.81&0.205&2.4&\\
%         \textbf{$\Delta$} & 1.0& 0.1& 0.1& 1.0& 1.0& 0.1& 0.1\\
%     \bottomrule
%     \end{tabular}
%     \caption{Domain-specific parameters for PDDL+ model repair in CartPole.}
%     \label{tab:cartpole_params}
% \end{table*}
\begin{figure*}[b]
    \centering
    \includegraphics[width=1\textwidth]{images/combined.pdf}
    \caption{Graphs showing performance of DQN-static/adaptive and planning-static/repairing agents. Episodes in a trial are on the x-axis and reward earned is shown on the y-axis. The results are averaged over $5$ trials. Red line indicates the episode where environment parameters were changed.}
    \label{fig:combined_results}
\end{figure*}

The planning agents were built with PDDL+. The expressiveness of PDDL+ enabled us to holistically encode CartPole's system dynamics as a planning domain (without using any external functions/solvers). Despite inherent complexity, efficient modeling allowed the use of off-the-shelf PDDL+ planners to solve the resulting problems. \roni{Maybe not say the previous sentence, as we say a bit later that we eventually did not do this} 
The planners were required to handle non-linear dynamics, large numbers of active happenings, and long temporal horizons. In our work on CartPole and other domains, we have successfully tested UPMurphi~\citep{della2009upmurphi} and ENHSP~\citep{scala2016interval}, but we ultimately opted for our own novel discretization-based PDDL+ planner \citep{matei2022system} that allows greater flexibility and customization (though, it relies on the same principles for solving PDDL+ problems as the other two planners). The planner solves full CartPole PDDL+ problems in approx. $0.1$ seconds using GBFS algorithm with a domain specific heuristic prioritizing ``safe" states (pole upright, low velocities, close to the center). We built two versions of the model-based planning agent. \emph{Planning-static} agent uses the same PDDL+ model for both the canonical and novelty setup. \emph{Planning-adaptive} agent monitors plan execution and automatically repairs the PDDL+ model inconsistency is detected as proposed in section \ref{sec:agent}. \emph{Repairable fluents} are all parameters defining CartPole dynamics (shown in Table \ref{tab:domain-paramaters}). Because, CartPole could be modeled exactly, Euclidean distance (from Section \ref{sec:inconsistency}) was used as a function for computing inconsistency $C$ with $C_{th}$ set to $0.01$. 

\subsubsection{Baseline Agents}
We compare model-based planning agents with reinforcement learning agents that are considered standard for the CartPole problem. Model-free RL agents were built with a standard deep Q-network implementation with experience replay memory \citep{mnih2013playing}. The Q-network is built with an input layer ($4 \times 16$), a hidden layer ($16 \times 16$), and an output layer ($16 \times 2$) and uses the Rectified Linear Unit (ReLU) activation function. The Q-network was trained to achieve perfect performance in the canonical setup, and is there difference between inconsistency for p prior to the experiments. The \emph{DQN-static} agent applies the policy learned in the canonical setup in the novelty setup. This baseline was implemented to ascertain that the introduced novelty indeed impacts performance of the agent and motivates adaptation. The \emph{DQN-adaptive} agent updated its network weights and learned a policy for the novelty setup.


\subsubsection{Results}
The performance of of all planning and model-free RL agents is summarized in Figure \ref{fig:combined_results}. The columns delineate the learning (DQN) v/s planning methods and the rows, their static and adaptive versions. In each graph, $x$-axis captures the episodes in a trial and the $y$-axis shows the total reward collected by the agent per episode, represented as the proportion of its score with a perfect controller. The red line indicates the episode where the selected novelty (shown in the graph title) was introduced. The shaded area represents the $95\%$ confidence interval computed over $5$ trials. 

As shown in Figure \ref{fig:combined_results}, all agents demonstrate perfect performance at the beginning of the trial and then experience a significant drop in performance as soon as the novelty is introduced (episode $8$). This drop demonstrates that the changes in the environment dynamics impacts the performance of all agents. There is variability in how each agent responds to the changes in the environment. We make the following observations:

\emph{Resilience of planning agents}: The novelty-induced performance drop is more significant in learning agents. For both types of novelties, the performance of the DQN agents drops below $30\%$ of its value in the canonical setup. In contrast, the performance of the planning agents drop to $\approx50\%$. This difference can be explained by the agents' design. The planning agents' PDDL+ model defines the system dynamics in a general manner. Thus, it can still be sufficiently accurate in some conditions. In contrast, the DQN agent's learned policy is not general and is only applicable for much reduced subset of cases after novelty.
    
\emph{Quick adaptation via model-space search}: As expected, after novelty is introduced, the static versions of the DQN and planning agents continue performing poorly, while the adaptive agents improve their performance over time. However, the time taken to improve differs greatly between the DQN-adaptive and planning-adaptive agents. Learning in DQN-adaptive is slow, requiring multiple interactions with the environment. In our experiments, DQN-adaptive took $\approx75$ episodes to reach $90\%$ of optimal performance as shown in Figure~\ref{fig:rl-long}. In contrast, the planning-adaptive agent recovers very quickly in $<20$ episodes for both novelties (Figure ~\ref{fig:combined_results}). This observation supports our central thesis: model-space search enables quick adaptation in dynamic environments because it can localize the learning to specific parts of the explicit model. Other parts of the explicit model are directly \emph{transferred} to the novel setup. Such transfer of knowledge is challenging to implement in end-to-end models such as DQNs in which action selection knowledge is distributed through the network.

Additionally, repair-based adaptation is scalable and can handle novelties that change system dynamics drastically from the canonical setup. Figure ~\ref{fig:repairing-gravity-20}) shows the planning-adaptive agent adapting to a novelty that changes gravity by a factor of more than two. As shown previously, planning-adaptive agents is able to accommodate this novelty in $\approx 17$ episodes.

\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.45\columnwidth}
         \centering
         \includegraphics[width=1\textwidth]{images/rl_masscart_9_long.png}
         \caption{Number of episodes needed by DQN-adaptive agent to learn a new policy for the novelty setup {length=1.1, masscart=0.9}}
         \label{fig:rl-long}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\columnwidth}
         \centering
         \includegraphics[width=1\textwidth]{images/repairing_gravity_20.png}
         \caption{Number of episodes needed by the planning-adaptive agent to learn to act in the novelty setup {length=1.1, gravity=20}}
         \label{fig:repairing-gravity-20}
     \end{subfigure}
     \caption{Additional adaptation results for model-free (a) and model-based (b) approaches}
     \vspace{0.5cm}
\end{figure}
    
    
\emph{Interpretable by design}: The model repair mechanism proposes specific and localized changes to the agent's explicit PDDL+ model. Thus, adaptation in the planning-adaptive agent is \emph{interpretable}. A model designer can inspect the proposed repair to understand why and how the novelty affected the agent's behavior. In contrast, learning in model-free systems such as DQN-adaptive cannot be interpreted directly. The following text shows the distinct repairs that were found by the planning-repairing agent using the method proposed in this paper. The reported values are changes from the nominal values used in the model. 

\begin{framed}
% \begin{console}
\small
     \noindent\textbf{Repair 1:} {mass\_cart: 0, length\_pole: 0.3, mass\_pole: 0, force\_mag: 0, gravity: 0, angle\_limit: 0, x\_limit: 0} \\
    \textbf{Repair 2:} {mass\_cart: 0, length\_pole: 0, mass\_pole: 0, force\_mag: 0, gravity: 1.0, angle\_limit: 0, x\_limit: 0}
    \\
    \textbf{Repair 3:} {mass\_cart: 0, length\_pole: -0.1, mass\_pole: -0.1, force\_mag: -1.0, gravity: 0, angle\_limit: 0, x\_limit: 0}
% \end{console} 
\end{framed}
\smallskip

Our method can find several distinct repairs that are not the `true' novelty i.e. the changes that are made in the environments transition model. However, the agent's performance converges to optimal with each one. This observation suggests that there are equivalence classes in the set of environmental parameters and their values. The agent uses only its observations over few episodes in the environment to guide its search for the correct model. The observations by themselves do not provide sufficient information to determine the parameter values exactly and can only differentiate between equivalence classes. These classes correspond to the ambiguity groups in model-based diagnosis. An analytical analysis of equivalence classes in CartPole parameters is out-of-scope for this paper.

\subsection{Angry Birds}
% Our next evaluation was done on ScienceBirds - a research variant of the popular game of Angry Birds. [roni: already said this above]
Our second set of experiments were conducted on Angry Birds and were designed to evaluate if the proposed repair mechanism can alleviate modeling inaccuracies by leveraging information gathered during agent run time. The objective in Angry Birds is to destroy pigs by launching birds at them from a sling-shot (shown in Figure \ref{fig:ab_level}). The launched birds obey the laws of motion and gravity. It is a difficult problem as it requires predicting outcomes of physics-based actions without having complete knowledge of the world, and then selecting an appropriate action out of infinitely many possible options. An Angry Birds level is \emph{passed} when all the pigs have been destroyed. Our tests were conducted in a specific subset of Science Birds levels containing a small number of birds, blocks, and pigs (a sample is shown in Figure \ref{fig:ab_level}). The goal of this experiment was to evaluate if the proposed method could alleviate inaccuracies in domain modeling during agent design.
\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{images/sb_level.png}
    \caption{A example of an Angry Birds level used in our experiments}
    \label{fig:ab_level}
\end{figure}
% \begin{table*}[h]
%     \centering
%     \begin{tabular}{l|ccccc}
%     \toprule
%         \textbf{repairable fluents} & \texttt{bird velocity}& \texttt{gravity}& \texttt{wood block multiplier}& \texttt{ice block multiplier}& \texttt{stone block multiplier}\\
%         \textbf{nominal values} & &&&&\\
%         $\Delta$ & $50.0$ & $1.0$ & $1.0$ & $1.0$ & $1.0$ \\
%     \bottomrule
%     \end{tabular}
%     \caption{Domain-specific parameters for PDDL+ model repair in ScienceBirds}
%     \label{tab:sb_params}
% \end{table*}


\subsubsection{Experiments} We conducted $11$ trials of $25$ levels each. To simulate inaccuracies in modeling that invariably creep in during model design phase, we deliberately encoded incorrect values for certain parameters in the agents.     Specifically, we reduced the maximum bird velocity by $4$ from its canonical value of $v_{bird}=186$. We measured how frequently each agent passes levels in a trial or the \emph{win rate}. The minimum possible win rate is $0$ (when no level in a trial is passed) and the maximum is $25$ (when all levels are passed).


\subsubsection{Planning Agent}
Following previous work on modeling Angry Birds with PDDL+ \citep{piotrowski2018heuristics}, we implemented a competent \emph{planning-static} agent. The PDDL+ model includes dynamics of launching a bird at maximum velocity at a certain angle, motion of birds and blocks, collisions between various objects, etc. 
While our PDDL+ model is accurate enough to plan effectively, it is not perfect. 
This issue manifests itself when computing inconsistencies between expected and observed trajectories. 
To address this we use an expanded inconsistency distance function, which considers not only the Euclidean distance between the expected and observed trajectories of thrown birds, but also counts any mismatch between the number of blocks that have not been broken at the end of each shot. The \emph{planning-adaptive} agent in this domain uses this new distance function to choose when to initiate repair of the PDDL+ model. We selected a subset of fluents in the model as \emph{reparable} (details in Table \ref{tab:domain-paramaters}) and set the consistency threshold $C_{th} = 50$. \johan{***** Johan: You haven't given the new function, so this threshold means nothing}.

\subsubsection{Results} 
We report the mean win rate for each agent and the $95\%$ confidence interval. The planning-static agent scored $0\% (0\%, 0\%)$ showing that the inaccuracy introduced in the model drastically degraded its performance. In contrast, the planning-adaptive agent scored $52.36\% (28.72\%, 75.96\%)$. These results indicate that the proposed repair mechanism can alleviate inaccuracies in the agent's model and improve its performance significantly.

The evaluations presented in this section demonstrate that learning by model repair leverages the strengths of using a compositional, white-box, planning model, and makes them robust to a class of domain shifts - novelties in open worlds - and modeling inaccuracies. Further, the paper proposes a formulation of inconsistency and search-based repair that are mostly \emph{domain-independent}. Indeed, we use the same implementation of repair for both CartPole and Angry Birds agents. Some domain specific knowledge (listed in Table \ref{tab:domain-paramaters}) is needed to structure and guide the search-based repair process. However, this knowledge is minimal and can be easily produced from the PDDL+ models implemented for each domain. \johan{***** Johan: Super weird thing to say, because if it was easy why did you not do it.}



\subsubsection{Result from Reward Divergence}
%Sookyung
In order to demonstrate the utility of the reward divergence score introduced in Section~\ref{sec:reward_divergence}, we present results of novelty detection using this score in the ScienceBirds environment. We first trained the reward estimation model ($g$). From approximately 15,000 data collected from a non-novel ScienceBirds environment, we use 80$\%$ for training and 20$\%$ for testing. We then evaluated the reward divergence score ($R_{div}$) in the ScienceBirds environment with Phase-3 novelties. To train the reward estimator, we normalized the scale of the input (state and action) and output (reward) to fall within a range between 0 and 1. The root mean square error (RMSE) score of the fully-trained reward estimator ($g^*$) tested in the non-novel environment was 0.008, indicating that the reward estimator is able to effectively predict rewards in a non-novel level. Given the fully trained reward estimator, $g^*$, the computed reward divergence scores, $R_{div}$, in Phase 3 the novelties are shown in Table~\ref{tab:results_reward_divergenece}. 
\roni{The reader is likely not from SAIL-ON project. What is Phase 3 is not clear to them. Why are we using SAI-ON codes?} 
As demonstrated in Table~\ref{tab:results_reward_divergenece}, levels 36-37 exhibit a higher reward divergence score compared to level 38. This aligns with the observation that levels 36-37 contain novelties that directly affect the reward, such as changes in gravity and the introduction of new objects or areas that have a direct impact on the reward. 

We also present the results of a binary classification task for detecting novelty from non-novelty using 600 test data, which was a mixture of 50$\%$ non-novel data and 50$\%$ novel data. To accomplish this, we utilized a pre-trained reward estimator (denoted as $g^*$) and computed RMSE score for each data point in the test set. Data points were classified as novel if their RMSE score was larger than a pre-defined threshold, and as non-novel otherwise. By varying the threshold between 0 and 1, we report True Positive Rates (TPR) and False Positive Rates (FPR).
Figure~\ref{fig:sb_precision_recall} illustrates the ROC curve for our novelty detection task, which was performed at different novelty levels and types, demonstrating the trade-off between TPR and FPR for various RMSE thresholds. Due to the multi-modality of reward distribution in the ScienceBirds environment, the ROC curve for the novelty detection task is quantized. As shown in the results, the novelty detection at level 36, type 1op11, exhibits the highest score of the area under the curve (AUC). This can be attributed to novelty from the gravity changes for birds, which causes a large divergence in rewards and makes it easier to detect novelty.


%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table*}[h!]
 \centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Level} & \textbf{Type} & \textbf{Reward Divergence  ($R_{div}$)}\\ \hline
36    & 10   & 0.4978                  \\
      & 11   & 0.4507                  \\
      & 12   & 0.5378                  \\
      & 13   & 0.4241                  \\
      & 14   & 0.4463                  \\
      & 20   & 0.5097                  \\
      & 21   & 0.0275                  \\
      & 22   & 0.4933                  \\
      & 23   & 0.5623                  \\
      & 24   & 0.4354                  \\ \hline
37    & 10   & 0.3357                  \\
      & 20   & 0.3869                  \\ \hline
38    & 14   & 0.0256                  \\
      & 20   & 0.0425                  \\
      & 21   & 0.0499                  \\
      & 22   & 0.0304                  \\
      & 23   & 0.0335                  \\
      & 24   & 0.0239                  \\ \hline
\end{tabular}
\caption{Reward divergence scores computed in Phase 3 novelties of ScienceBirds \roni{Can we relate the results to known detection metrics? (accuracy, precision, recall)}}\label{tab:results_reward_divergenece}
\end{table*}



\begin{figure*}[h!]
\centering
\includegraphics[width=.49\textwidth]{images/roc_level36type10-14.png}
\hfill
\includegraphics[width=.49\textwidth]{images/roc_level36_type20-24.png}

\includegraphics[width=.49\textwidth]{images/roc_level37.png}\hfill
\includegraphics[width=.49\textwidth]{images/roc_level38.png}
\caption{Precision-recall curves of the novelty detection task using ScienceBirds environment with novelty level 36, 37 and 38. }
\label{fig:sb_precision_recall}
\end{figure*}
%%%%%%%%%%%%%%%%%%


==> extra_text.tex <==
\section{Background}
The approach proposed in this paper is best suited for planning agents built with domain-independent planning algorithms operating on domain-specific models (including various levels of PDDL \citep{mcdermott1998pddl}, i.e, PDDL2.1~\citep{fox2003pddl2}, PDDL+ \citep{fox2006modelling} etc). PDDL+ has been previously used to model a range of complex planning problems, including Chemical Batch Plant~\citep{della2010pddl+}, Atmospheric Reentry~\citep{piotrowski2018heuristics}, Urban Traffic Control~\citep{vallati2016efficient}, and Planetary Lander~\citep{della2010resource}. 

PDDL+ is suited for a broad range of applications that feature a world with discrete and continuous state variables, exogenous activity, and non-linear system dynamics. Situating our research in PDDL+ enables us to study open-world learning in scenarios that embody the complexity in real-world environments. Our approach can be applied to classical planning agents operating in discrete world through minor modifications. 

==> old-hydra.tex <==
\section{HYDRA}
\label{sec:hydra}

The main contribution of this work is the design of HYDRA, a domain-independent architecture for implementing a novelty-aware agent in complex, mixed discrete and continuous domains.  
A HYDRA agent implements a meta-reasoning framework that detects and adapts to novelties. 
A notional architecture is shown in Figure \ref{fig:hydra_architecture}. The architecture consists of a \emph{base agent} augmented with  \emph{novelty meta-reasoning} components designed to detect and adapt to novelties. 


The base agent (Figure \ref{fig:hydra_architecture} - left) implements a  \emph{perceive-decide-act} cycle in the environment, inferring the current state of the world using encoded background knowledge and perceived observations, deciding which actions to perform using a PDDL+ planner, and acting accordingly. 
The main components in the base agent are the state inference component, the task selection component, and the planning component. These components map to the well-known Belief-Desire-Intention elements in the BDI agent architecture~\cite{georgeff1999belief}, and connect the domain-specific aspects of the problem to the domain-independent mechanisms.  


The novelty meta-reasoning components consist of a set of \emph{novelty monitors} that maintain a variety of explicit expectations about the environment evolution and monitor divergence; a \emph{novelty detection} component that aggregates the information from the monitors
and determines if a novelty has been introduced and requires adaptation; and finally, a \emph{heuristic search-based model repair} component that manipulates  the base agent's PDDL+ model to the detected novelty. 
Next, we describe in more detail our implementation of the main HYDRA  components. 

% The main components in the base agent (Figure \ref{fig:hydra_architecture} - left) are the state inference component, the task selection component, and the planning component. These components map to the well-known Belief-Desire-Intention elements in the BDI agent architecture~\cite{georgeff1999belief}, and connect the domain-specific aspects of the problem to the domain-independent mechanisms.  




% HYDRA has been tested with three domains: CartPole++ (a three dimensional variation of the classic control problem - CartPole), Science Birds (an AI competition domain), and PogoStick (a minecraft domain) and can be extended to mixed discrete-continuous environments.\roni{This repeats the above. We already say this in the introduction and problem setup}

% HYDRA implements a meta-reasoning framework that detects,  characterizes, and accommodates novelties. A notional architecture is shown in Figure \ref{fig:hydra_architecture}. The architecture consists of a \emph{base agent} that implements the perceive-decide-act cycle in the environment. It uses planning models written in PDDL+ to determine a sequence of actions. To reason about novelty, HYDRA implements a \emph{meta reasoning} process that adapts the models in the base agent. The process consists of a set of \emph{novelty monitors} that maintain a variety of explicit expectations about the environment evolution and monitor divergence; \emph{novelty inference} that determines if there is novelty in the environment based on information from the monitors; and finally, a heuristic search-based model repair for novelty accommodation that adapts the PDDL+ models to work in the novel setup. HYDRA has been tested with three domains: CartPole++ (a three dimensional variation of the classic control problem - CartPole), Science Birds (an AI competition domain), and PogoStick (a minecraft domain) and can be extended to mixed discrete-continuous environments.

% HYDRA is a domain-independent architecture for implementing model-based reasoning agents that are \emph{novelty-aware} - it implements a meta-reasoning framework that detects, characterizes, and accommodates novelties. A notional architecture is shown in Figure \ref{fig:hydra_architecture}. The architecture consists of a \emph{base agent} that implements the perceive-decide-act cycle in the environment. It uses planning models written in PDDL+ to determine a sequence of actions. To reason about novelty, HYDRA implements a \emph{meta reasoning} process that adapts the models in the base agent. The process consists of a set of \emph{novelty monitors} that maintain a variety of explicit expectations about the environment evolution and monitor divergence; \emph{novelty inference} that determines if there is novelty in the environment based on information from the monitors; and finally, a heuristic search-based model repair for novelty accommodation that adapts the PDDL+ models to work in the novel setup. HYDRA has been tested with three domains: CartPole++ (a three dimensional variation of the classic control problem - CartPole), Science Birds (an AI competition domain), and PogoStick (a minecraft domain) and can be extended to mixed discrete-continuous environments.

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{images/hydra_architecture.png}
    \caption{HYDRA - a domain-independent architecture for novelty reasoning}
    \label{fig:hydra_architecture}
\end{figure}

% \subsection{Base Agent}
% \label{sec:base-agent}


\subsection{State Inference}
The role of this HYDRA component is to infer the current state of the environment in sufficient detail to enable symbolic task selection and planning. Different environments provide a variety of input signals including visual information (images, object detection and colormap in ScienceBirds), continuous-valued sensor information (position and velocity of the cart and the pole in CartPole-3D), as well as discrete state information (locations and positions in PogoStick).


The HYDRA \emph{visual reasoning} component is responsible for performing the required image processing needed to extract symbolic information from the provided visual information. 
As each domain may structure its visual input differently, the HYDRA visual reasoning component requires a domain-specific recognition model that detects, localizes, and categorizes known objects and their properties in the input. 

The HYDRA \emph{state inference}  component accepts the symbolic information about the current state obtained either via the visual reasoning component or directly from the environment and integrates it with a-priori knowledge about the domain and the current state. This process is largely domain-dependent and is also known as belief update. 

\begin{example}
In the ScienceBirds domain, the HYDRA visual reasoning component accepts a set of visible objects on the scene including their locations and a vector representing their visual structures. The vector consists of the number of vertices in the bounding polygon, the area of the bounding polygon, as well as the a list of compressed 8-bit (RRRGGGBB) color and their percentage in the object. The HYDRA visual reasoning component for Science Birds accepts such vectors as input and categorizes the object as one of the known object classes. This was done using a standard implementation of multinomial logistic regression for multi-class classification., 
using a dataset of $13198$ datapoints obtained by sampling ScienceBirds levels. Importantly, this training was performed in a pre-processing stage, before novelties have been introduced.
The state inference component adds to this symbolic information the current assumption about the number of health points each pig and block have, which also considers historical data about how many times each object has been hit by previous shots. 
\end{example}

% This mapping of symbolic information to PDDL+ terminology is also domain-dependent, and includes adding a-prior knowledge about the domain. For example, in Polycraft the HYDRA state inference component translates the number of diamonds in the inventory to a corresponding PDDL+ numeric fluent (these called \emph{functions} in PDDL+). 
% In ScienceBirds, the state inference component also includes our current assumption about the number of health points each pig has. 








% For example, in the ScienceBirds domain, the HYDRA visual reasoning component accepts a set of visible objects on the scene including their locations and a vector representing their visual structures. The vector consists of the number of vertices in the bounding polygon, the area of the bounding polygon, as well as the a list of compressed 8-bit (RRRGGGBB) color and their percentage in the object. The HYDRA visual reasoning component for Science Birds accepts such vectors as input and categorizes the object as one of the known object classes. This was done using a standard implementation of multinomial logistic regression for multi-class classification., 
% using a dataset of $13198$ datapoints obtained by sampling ScienceBirds levels. Importantly, this training was performed in a pre-processing stage, before novelties have been introduced.



% create a PDDL+ domain and problem representing the environment dynamics and its current state, respectively, which can be used by a PDDL+ planner to determine the next actions to perform. 
% As input, the state inference HYDRA component accepts the symbolic information about the current state obtained from the environment (possibly via the visual reasoning component). 
% This mapping of symbolic information to PDDL+ terminology is also domain-dependent, and includes adding a-prior knowledge about the domain. For example, in Polycraft the HYDRA state inference component translates the number of diamonds in the inventory to a corresponding PDDL+ numeric fluent (these called \emph{functions} in PDDL+). 
% In ScienceBirds, the state inference component also includes our current assumption about the number of health points each pig has. 

% The base agent begins with processing observations provided by the environment. Different environments provide a variety of input signals including visual information (images, object detection and colormap in ScienceBirds), continuous valued sensor information (position and velocity of the cart and the pole in CartPole-3D), as well as discrete state information (locations and positions in PogoStick).



% \paragraph{Visual Reasoning} In some domains, the observations collected by HYDRA are visual. 
% For these domains, HYDRA performs visual reasoning to extract symbolic information from the provided visual information. 
% As each domain may structure its visual input differently, HYDRA requires a domain-specific recognition model that detects, localizes, and categorizes known objects and their properties in the input. 
% For example, in the ScienceBirds domain, the HYDRA visual reasoning component accepts a set of visible objects on the scene including their locations and a vector representing their visual structures. The vector consists of the number of vertices in the bounding polygon, the area of the bounding polygon, as well as the a list of compressed 8-bit (RRRGGGBB) color and their percentage in the object. The HYDRA visual reasoning component for Science Birds accepts such vectors as input and categorizes the object as one of the known object classes. This was done using a standard implementation of multinomial logistic regression for multi-class classification., 
% using a dataset of $13198$ datapoints obtained by sampling ScienceBirds levels. Importantly, this training was performed in a pre-processing stage, before novelties have been introduced. 

% The dataset consists of $13198$ datapoints obtained by sampling ScienceBirds levels implementing the canonical, non-novel setup. The datapoints represent $13$ distinct object classes that are in HYDRA's domain ontology for ScienceBirds. Table \ref{tab:sb_classification} shows the accuracy of the model in a $20\%$ test set, showing that the model can reliably categorize all relevant objects.


% The ScienceBirds domain provides a set of visible objects on the scene including their locations as well as a vector representing their visual structures. The vector consists of the number of vertices in the bounding polygon, the area of the bounding polygon, as well as the a list of compressed 8-bit (RRRGGGBB) color and their percentage in the object. A recognition module was designed that accepts this vector as an input and categorizes the object as one of the known object classes. 

% The Science Birds recognition module has been built with a standard implementation of multinomial logistic regression for multi-class classification. The dataset consists of $13198$ datapoints obtained by sampling ScienceBirds levels implementing the canonical, non-novel setup. The datapoints represent $13$ distinct object classes that are in HYDRA's domain ontology for ScienceBirds. Table \ref{tab:sb_classification} shows the accuracy of the model in a $20\%$ test set, showing that the model can reliably categorize all relevant objects.

% \begin{table}[]
% \centering
% \begin{tabular}{llll}
% Class      & Precision & Recall & F1-score \\
% TNT        & 1.0       & 1.0    & 1.0      \\
% butterfly  & 1.0       & 1.0    & 1.0      \\
% ice        & 1.0       & 1.0    & 1.0      \\
% magician   & 1.0       & 1.0    & 1.0      \\
% pig        & 1.0       & 1.0    & 1.0      \\
% platform   & 1.0       & 1.0    & 1.0      \\
% redBird    & 1.0       & 1.0    & 1.0      \\
% slingshot  & 1.0       & 1.0    & 1.0      \\
% stone      & 1.0       & 1.0    & 1.0      \\
% wizard     & 1.0       & 1.0    & 1.0      \\
% wood       & 1.0       & 1.0    & 1.0      \\
% worm       & 1.0       & 1.0    & 1.0      \\
% yellowBird & 1.0       & 1.0    & 1.0      \\
% \hline
% accuracy   &           &        & 1.0     
% \end{tabular}
% \caption{\roni{What is the point of showing this table if it's all ones? we can just say that it's perfect in the non-novel case.}}
% \end{table}
% \label{tab:sb_classification}

% \paragraph{State Inference}
% The role of this HYDRA component is to create a PDDL+ domain and problem representing the environment dynamics and its current state, respectively, which can be used by a PDDL+ planner to determine the next actions to perform. 
% As input, the state inference HYDRA component accepts the symbolic information about the current state obtained from the environment (possibly via the visual reasoning component). 
% This mapping of symbolic information to PDDL+ terminology is also domain-dependent, and includes adding a-prior knowledge about the domain. For example, in Polycraft the HYDRA state inference component translates the number of diamonds in the inventory to a corresponding PDDL+ numeric fluent (these called \emph{functions} in PDDL+). 
% In ScienceBirds, the state inference component also includes our current assumption about the number of health points each pig has. 



% \roni{Anyone knows what this is intended to have?}
% \roni{I get it now: how to add the background knowledge. TODO for me to explain}
% \roni{TODO For me: make this section domain-independent - only partially done}

\subsection{Task Selection}
%%% Roni Stern and Sachin Grover please complete this section.

The main task for the HYDRA agent is based on the domain, such as, to craft a pogostick in PogoStick or kill all the pigs in ScienceBirds domain. 
Planning directly towards achieving this task is possible in some domains, while in other domains it is necessary or more efficient to select intermediate tasks (also referred to as subtasks) for the agent to achieve as steps towards achieving its main task. 
The HYDRA task selection component implements this subtask mechanism, as follows.


Implementing a HYDRA agent for a given domain requires defining one or more HYDRA tasks.  
A \emph{HYDRA task} is a tuple $\tau=\tuple{\pre_\tau, \mathcal{D}_\tau, G_\tau}$ 
representing the preconditions, domain, and goal of the task. 
The preconditions of a task ($\pre_\tau$) define when performing this task may be useful, and the goal of a task ($G_\tau$) defines what this task aims to achieve.  
The domain of a task ($\mathcal{D}_\tau$) is a subset of the HYDRA agent domain $\mathcal{D}$ specifies the parts of the domain relevant for performing the task. This is useful for efficiency reasons: performing some tasks do not require reasoning about all aspects of the domain. 




A HYDRA task is \emph{relevant} if its preconditions ($\pre_\tau$) are met and its goal ($G_\tau$) has not been achieved yet. 
The HYDRA agent maintains a set of relevant HYDRA tasks and designates one of these tasks as the \emph{active task}. 
This is the task the HYDRA agent is currently aiming to achieve. 
HYDRA calls the task selection component to consider changing the active task if the current task is no longer relevant or a performed action had unexpected outcomes. Then, it uses domain-specific decision rules to decide if the active task should be replaced and if so, which of the relevant tasks should be set as the new active task. 
Note that some of the relevant tasks may be exploration tasks, whose preconditions relate to detected novelties. 

\begin{example}
Task selection in non-novel environments for Science Birds and Cartpole++ is trivial, including a single task to achieve the corresponding domain's goal (kill all birds or maintain the pole's upright angles). 
A richer task selection component was implemented for PogoStick, since the environment has additional agents that may interfere with the base agent's plans, 
and includes objects such as a safe or a chest, whose content is unknown and may have useful resources. 
Thus, the HYDRA agent for PogoStick includes exploratory tasks designed to gather information that might help craft the pogo stick more efficiently.
Specifically, the tasks in our implementation of HYDRA for this domain include:
\begin{itemize}
    \item [$(\tau_1)$] Craft a pogo stick
    \item [$(\tau_2)$] Interact with other agents.
    \item [$(\tau_3)$] Explore other rooms.
    \item [$(\tau_4)$] Open a safe or a chest.
    \item [$(\tau_5)$] Attempt to mine novel objects.
\end{itemize}
$\tau_1$ is the main task of the game. 
$\tau_2$ includes interacting with trader agents to learn the trade recipes they support. A trade recipe can be, for example, trading 9 diamonds for 1 titanium. 
This task is necessary because some items required for crafting the pogo stick can only be obtained by trading with these trader agents. 
The domain of task $\tau_2$ is very limited, including only the location of the other agents and obstacles that may block getting to them, while the domain of task $\tau_1$ additional information such as crafting recipes. 


Tasks $\tau_1$ and $\tau_2$ are usually sufficient to solve the problem in non-novelty environments. 
Thus, the task selection decision rules used for this domain selects these tasks first, and only select the other tasks ($\tau_3, \tau_4, \tau_5$) after $\tau_1$ and $\tau_2$ was selected and in case where we failed to craft the pogo stick. Between these tasks, we selected the tasks in the sequential order they are presented, i.e., try $\tau_3$ first, then $\tau_4$, and finally $\tau_5$.
\end{example}



% The intermediate task selected by this component is used to define the goal, construct a plan of action and execution. 



\subsection{Planning and Execution}
HYDRA leverages a PDDL+ planner to determine a sequence of actions given the active task and the current state.  
It translates the domain of the active task and the current state into PDDL+. 
The current state is represented as a set of grounded predicates and functions (discrete and numeric state variables). 
The richness of PDDL+ enables direct encoding of the active task's domain, supporting the definition of actions, events, and durative processes.\footnote{The effects of processes and events are implicitly applied via a time-passing action that the agent can apply alongside the actions defined in the PDDL+ domain.}. Each happening is represented as a pair of \emph{pre-conditions} and \emph{effects} expressed in terms of assignments and mathematical expressions. 


The PDDL+ planner outputs a sequence of actions for the agent to perform. HYDRA maintains this plan and attempts to execute it. If an action fails, we halt the execution and call the task selection component to consider changing the active task, or replanning for the current active task. Identifying action failure is done by analyzing feedback from the environment, and comparing with the expected outcome of each action as defined by the domain. 


\begin{example}
An example of a process from the CartPole++ domain is shown in Figure \ref{fig:process-cartpole}. A planning \emph{problem} $\mathcal{P}$ in the domain $D$ is a pair $\mathcal{P}=\tuple{s_0,G}$ where $s_0\in S$ is the initial state., and $G \subseteq S$ is a set of possible goal states. A solution to a problem $\mathcal{P}$ is a plan $\pi = (a_0, a_1, ..., a_n)$ which reaches a goal state $s_G \in G$. Executing a plan $\pi$ in domain $D$ yields a trajectory $\tau = (\tuple{s_0, a_0, s_1}, \tuple{s_1, a_1, s_2}, ... , \tuple{s_n, a_n, s_G})$, which comprises a sequence of tuples of the form $\tuple{s_i, a_i, s_{i+1}}$, representing that the agent performed action $a_i$ in state $s_i$, and reached state $s_{i+1}$.
\end{example}


% HYDRA leverages a PDDL+ planner to determine a sequence of actions given the active task and the current state.  
% It translates the domain of the active task and the current state into PDDL+. 
% The current state is represented as a set of grounded predicates and functions (discrete and numeric state variables). 
% To plan, domain $D$ is the agent's internal approximation of environment $E$, defining how the state changes under various \emph{happenings} that include actions, events that were triggered, and durative processes that are may be active\footnote{The effects of processes and events are implicitly applied via a time-passing action that the agent can apply alongside the actions defined in the PDDL+ domain.}. Each happening is represented as a pair of \emph{pre-conditions} and \emph{effects} expressed in terms of assignments and mathematical expressions. An example of a process from the CartPole++ domain is shown in Figure \ref{fig:process-cartpole}. A planning \emph{problem} $\mathcal{P}$ in the domain $D$ is a pair $\mathcal{P}=\tuple{s_0,G}$ where $s_0\in S$ is the initial state., and $G \subseteq S$ is a set of possible goal states. A solution to a problem $\mathcal{P}$ is a plan $\pi = (a_0, a_1, ..., a_n)$ which reaches a goal state $s_G \in G$. Executing a plan $\pi$ in domain $D$ yields a trajectory $\tau = (\tuple{s_0, a_0, s_1}, \tuple{s_1, a_1, s_2}, ... , \tuple{s_n, a_n, s_G})$, which comprises a sequence of tuples of the form $\tuple{s_i, a_i, s_{i+1}}$, representing that the agent performed action $a_i$ in state $s_i$, and reached state $s_{i+1}$.


\begin{figure}
\centering	
% \begingroup
\fontsize{8pt}{10pt}\selectfont
\begin{verbatim}
    (:process movement
    :parameters ()
    :precondition (and (ready)(not (total_failure)))
    :effect (and (increase (x) (* #t (x_dot)) )
    (increase (theta) (* #t (theta_dot)))
    (increase (x_dot) (* #t (x_ddot)) )
    (increase (theta_dot) (* #t (theta_ddot)) )
    (increase (elapsed_time) (* #t 1) ) ))
\end{verbatim}
% \endgroup
\caption{Continuous PDDL+ process updating over time the positions and velocities of the cart and pole in CartPole++.}
\label{fig:process-cartpole}

\end{figure}


\subsection{Novelty Monitors}
\label{sec:monitors}
HYDRA implements a set of monitors that observe various aspects of agent behavior in its environment and compute how divergent 


\roni{What's supposed to be here?}
\subsubsection{Unknown Elements}
\roni{What's supposed to be here?}

\subsubsection{Reward Divergence} \label{sec:reward_divergence}
%%% Sookyung Kim

The reward divergence score for any modeled domain $D$ and a plan $\tau$, denoted as $R_{div}(D,\tau) \in \mathbb{R}_{\ge 0}$, \roni{What is $D$ and what is $\tau$} is a metric that quantifies the extent to which the reward diverges in an environment containing a novelty in comparison to a non-novel environment, when the same actions are taken in the same states. 
\roni{Need to explain here that we cannot compute it because we cannot perform the same action in the same state in novel and non-novel environments because the novelty might have also changed the states themselves. Right? therefore, we rely on these function approximations }
To calculate this score in a data-driven manner, we developed a neural-network-based prediction model, denoted as $g$, that estimates the reward in a non-novel environment, denoted as $r_i$, given the input of the state, $s_i$, and the action, $a_i$. Mathematically, this can be represented as:

\begin{align}
  \mathbf{\widehat{r}}_{i}
  & = g(s_i, a_i) \nonumber\\
  & \approx \arg\max_{\mathbf{r}_i} p(\mathbf{r}_i | s_i, a_i).
\end{align}
To train the model $g$, we minimize the root mean squared loss ($\mathcal{L}$) between the estimated reward $\hat{r}_{i}$ from model $g$ and the ground-truth reward $r_{i}$, through the following optimization problem:

\begin{equation}
 \mathcal{L}= \min_{\Theta} \sqrt{\frac{1}{N} \sum_{i=1}^{N}  \|\hat{\mathbf{r}}_i - \mathbf{r}_i\|_2^2},
\end{equation}

Where $N$ is the number of training data points and $\Theta$ is the set of parameters in our models $g$. To demonstrate the reward estimation model, we apply it to the domain of ScienceBirds. Since the state $s_i$ in ScienceBirds can be represented as a visual scene composed of multiple channels of different objects, we utilize Convolutional Neural Networks (CNNs) for $g$, which have been proven to be successful in learning visual representations. The architecture of the reward estimator model for ScienceBirds is illustrated in Figure~\ref{fig:reward_estimator}.
%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=13.5cm]{images/reward_estimator.png}
\end{center}
\caption{Model architecture of the reward estimator for ScienceBirds}
\label{fig:reward_estimator}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%

Our training set consists of approximately 15,000 data points of state-action pairs $)(s_i, a_i)$, labeled with corresponding rewards $r_i$, collected from a non-novel ScienceBirds environment. By fully pre-training the reward estimation model with this non-novelty dataset, $g^*$ learns to map from the state-action pair to the expected reward assuming an environment is non-novel. Therefore, when we introduce novelty, the error between the reward estimated from $g^*$ and the ground truth reward represents the reward divergence between the expected reward in a non-novel environment ($g^*(s_i, a_i)$) and the actual reward in a novel environment ($r_i$).

Consequently, the reward divergence score $R_{div}$ due to a novelty is computed as the root mean squared error between the predicted reward from $g^*$ and the ground truth reward $r$, mathematically represented as:

\begin{equation}
 R_{div}(D, \tau) = \sqrt{\frac{1}{\|\tau\|} \sum_{i=1}^{\|\tau\|}  \|g^*(s_i, a_i) - \mathbf{r}_i\|_2^2},
\end{equation}

where $\tau$ is a trajectory collected in a novel environment, and $g^*$ is the reward-estimator pre-trained with dataset collected from a non-novel environment.  The magnitude of the reward divergence score, $R_{div}$, serves as an indicator of how much the reward deviates in an environment with a novel feature as compared to a non-novel environment, given identical actions taken in the same state. Thus, a larger value of $R_{div}$ implies a more pronounced deviation in reward, making the novelty present in an environment easily detectable.

\subsubsection{Inconsistency Computation \roni{Maybe Planning Model Inconsistency?}}
\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{images/trajectory_inconsistency2.png}
	\caption{Visualization of the inconsistency score (black, dashed line) of the expected state trajectory obtained from the plan generated with agent's internal model $D$ (pink nodes) with respect to the observations trajectory $\tau$ from the environment $E^*$ (green nodes).}
	\label{fig:inconsistency_trajectory}
\end{figure}
Inconsistency score $C(\pi, D, \tau) \in \mathbb{R}_{\ge 0}$ is a measure of how accurately the planning model $D$ describes the actual environment and its dynamics, when executing a plan $\pi$ starting in state $s$. It is computed using two aligned trajectories. 
The first trajectory is obtained by simulating\footnote{Plan simulation can be done using dedicated plan simulators such as VAL~\citep{howey2004val}. In our work, we wrote our own general-purpose PDDL+ simulator used across various domains.} the generated plan $\pi$ and the model $D$. The other trajectory $\tau$ is generated by the environment upon executing the plan $\pi$. 
Inconsistency score $C$ is the ``distance'' between pairs of corresponding states in simulated and observed trajectories discounted proportionally by time. 
There are many ways to measure this ``distance'', and the exact function can be domain-dependent. 
In this work, the distance is defined as the Euclidean distance between the pairs of corresponding states in the observed and expected trajectories. In the most general case, the distance would be calculated over all state variables $F \cup X$ (where propositional values are cast as 1 or 0). However, for increased accuracy, this can be restricted to a subset of relevant state variables.
% Inconsistency $C$ is the sum of Euclidean distances between pairs of corresponding states in simulated and observed trajectories discounted proportionally by time. 
Formally, let $S(\tau)$ be the sequence of states in the observed trajectory and $S(\pi,D)$ be the expected sequence of states obtained by simulating the generated plan $\pi$ with respect to the agent's internal model $D$. Let $S(x)[i]$ denote the $i^{th}$ state in the state sequence $S(x)$. Inconsistency score of domain $D$ is computed as:
\begin{equation}
    C(\pi, D, \tau) = \frac{1}{|\tau|} \sum_{i} \gamma^i\cdot ||S(\tau)[i] - S(\pi,D)[i]||
\end{equation}
where $0<\gamma<1$ is the discount factor. Errors in $C$ due to sensing noise, rounding errors, and other issues can accumulate over time. Consequently, the Euclidean distance between corresponding states is likely to be higher later in the trajectories. The discount factor $\gamma$ prevents such errors from dominating the inconsistency score.  

In a non-novel environment $E$ with an ideal domain $D$, the expected evolution of the system predicted by the planner should perfectly match the observed behavior in simulation, i.e., the two resulting trajectories align by default with the inconsistency score $C=0$. 
In the real world, however, this is usually impossible to achieve due to rounding errors, perception inaccuracies, and similar common issues. To account for such noise, a domain-specific consistency threshold $C_{th}$ is set. A model $D$ is inconsistent with $E^*$ ($D \ncong E^*$) if $C(\pi, D, \tau) \ge C_{th}$ and consistent otherwise. Setting $C_{th}$ requires striking a fine balance between accurately estimating the inconsistency score and suppressing noise stemming from the execution environment. 

A graphical representation of state trajectory-based inconsistency score computation is shown in Figure~\ref{fig:inconsistency_trajectory} in which the expected state trajectory under the agent's internal model $D$ (pink nodes) is compared against the observed trajectory (green nodes) in the environment $E$. The left y-axis denotes the Euclidean distance between states and the right y-axis, the inconsistency score. Due to the discount factor $\gamma$, the distance between states later in the trajectory contribute less to the inconsistency score than the distance between states earlier in the trajectory. The model is deemed inconsistent ($D \ncong E)$ if the inconsistency threshold is exceeded.

%\roni{I am concerned that this paper will be a superset of the IJCAI paper. If that's the case then it may be problematic.}

\subsection{Inference}
\textcolor{red}{Adding the environment based explanation for handling novelty and the flow diagram as the inference part. $\sim$ Sachin.}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{images/novelty-reasoning.png}
    \caption{Diagram of the agent's architecture for novelty reasoning. The solid lines denote classical planning setup $D \cong E$. 
    The dotted lines denote learning to operate in a novel world by revising model such that $D^* \cong E^*$}
    \label{fig:novelty_reasoning}
    \vspace{-4mm}
\end{figure}

Figure \ref{fig:novelty_reasoning} shows the proposed novelty reasoning process for a planning agent.
Recall that initially $D$ models environment $E$, and in an episode unknown to the agent switches to $E^*$ due to introduction of novelty. The change in the environment is not known to the agent and can only be reasoned about based on observations.
\begin{enumerate}
    % \item At the beginning of an episode, the agent uses the data from the current state ($s_t$) and applies some domain-specific complementary assumptions about the environment to generate a problem ($s_t, G$). For example, in CartPole, the agent might observe specific positions of the cart and pole and apply assumptions about gravity and friction coefficient that govern movement. The problem is then paired with the domain $D$ hand-designed a-priori.
    \item At the beginning of an episode, the agent accepts the current state $s_t$ and creates a corresponding planning problem ($s_t, G$). This problem is then paired with the domain $D$, which was created a-priori.
    \item The agent uses a planner to solve the generated planning problem to obtain a feasible plan $\pi$. 
    \item The agent executes the plan $\pi$ in the environment. During execution, it stores the observed trajectory $\tau$ as a list of $\tuple{s_t,a,s_{t+1}}$ state transitions. 
    \item At the end of the episode, the agent computes the inconsistency score $C(\pi, D, \tau)$ for the current model $D$ by comparing the expected state trajectory (obtained by simulating plan $\pi$) with the observed execution trace, $\tau$ (elaborated in Section \ref{sec:inconsistency}).
    \item If the inconsistency score exceeds a set threshold $C_{th}$, the agent infers that $D \ncong E^*$, i.e, its model $D$ has become inconsistent with the current environment $E^*$. 
    \item The search-based model repair (elaborated in Section \ref{sec:repair}) is engaged to adjust the agent's internal domain model $D$. It searches through candidate repairs $D^*$ to find one which sufficiently reduces the inconsistency score. The result is an updated model $D^*$ whose inconsistency with the current environment $E^*$ lower than $D$.
    \item The agent moves on to the next episode and uses the updated domain model $D'$ to solve the subsequent tasks. %The whole process repeats again from the start (1.) and continues until the agent finds a model $D^* \cong T^*$ or $C(\pi, D^*, \tau) < C_{th}$.
\end{enumerate}

% Step X is the novelty detection in open-world learning and step Y is .....[some mix of these sentences]
% This step is novelty \emph{detection} in the open-world learning. 
% Identification of $D^*$ is the novelty \emph{characterization} and \emph{accommodation} in open-world learning. 
Step 5 above corresponds to novelty \emph{detection} in open-world learning. Step 6 corresponds to \emph{characterization} and \emph{accommodation} - the agent reasons about which element of its planning model should be adapted so that its expectations become consistent with observations. It takes a few repair steps ($5$ and $6$) for the agent to find a consistent domain model $D^* \cong E^*$ because a single trajectory may only provide enough information to find a partial repair.

For clarity, note that the planning domain describes general structure and system dynamics, and only needs to be defined once per environment. On the other hand, the planning problem is auto-generated per episode, combining the initial state data obtained from the environment and assumptions about the domain (i.e., values for variables that are required to accurately describe the environment and its dynamics, but which are not included in the data from the environment, e.g., gravity, velocities of moving entities).


\subsection{Heuristic Search-Based Repair}

The proposed search-based model repair algorithm works by searching for a \emph{domain repair} $\varPhi$, which is a sequence of model modifications that, when applied to the agent's internal domain $D$, returns a domain $D'$ that is consistent with the observed trajectories.
To find such a domain repair, our algorithm accepts as input a set possible basic \emph{Model Manipulation Operators} (MMOs), denoted $\{\varphi\} = \{\varphi_0, \varphi_1, ... , \varphi_n\}$. Each MMO $\varphi_i \in \{\varphi\}$ represents a possible change to the domain. Thus, a domain repair $\varPhi$ is a sequence of one or more basic MMO $\varphi_i \in \{\varphi\}$. An example of an MMO is to add a fixed amount $\Delta\in\mathbb{R}$ to one of the numeric domain fluents.
In general, one can define such an MMO for every domain fluent. In practice, however, not all domain fluents are equal in their importance thus the repair can be focused on a subset of state variables that the domain designer deems relevant.


\begin{algorithm}
% \fontsize{9pt}{7pt}\selectfont
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
% \SetKwComment{Comment}{$\triangleright$\ }{}
\Input{$\{\varphi\}$, a set of basic MMOs}
\Input{$D$, the original PDDL+ domain}
\Input{$\pi$, plan generated using $D$}
\Input{$\tau$, a trajectory}
\Input{$T$, consistency threshold}
\Output{$\varPhi_{best}$, a domain repair for $D$}
OPEN$\gets\{\emptyset\}$; 
$C_{best}\gets\infty$;
$\varphi_{best}\gets\emptyset$\\
\While{$C_{best}\geq T$}{
    $\varPhi\gets$ pop from OPEN\\
    \ForEach{$\varphi_i\in\{\varphi\}$}{
        $\varPhi'\gets \varPhi \cup \varphi_i$ {\scriptsize \tcc*{Compose a domain repair}} 
        DoRepair($\varPhi'$, $D$)\\
        $C_{\varPhi'}\gets$ InconsistencyEstimator($\pi$, $D$, $\tau$)\\
        \If{$C_\varPhi\leq C_{best}$}{
            $C_{best}\gets C_{\varPhi'}$\\
            $\varPhi_{best}\gets\varPhi'$
        }
        Insert $\varPhi'$ to OPEN with key $f(\varPhi', C_{\varPhi'})$ \nllabel{alg:line:f}\\
        UndoRepair($\varPhi'$, $D$)
    }
}
\Return $\varPhi_{best}$\\
\caption{PDDL+ general model repair algorithm.}
% \label{alg:repair}
\end{algorithm}


Algorithm~\ref{alg:repair} lists the pseudo-code for our search-based model repair algorithm. 
Initially, the open list ($OPEN$) includes a single node representing the empty repair, 
and the best repair seen so far $\varPhi_{best}$ is initialized to an empty sequence. 
This corresponds to not repairing the agent's internal domain at all. 
Then, in every iteration the best repair in OPEN is popped, and we compose new repairs by adding a single MMO to this repair, and add them to $OPEN$.  
For every such repair $\varPhi'$ we compute an inconsistency score $C_{\varPhi'}$. 
This is done by modifying the agent's internal domain $D$ with repair $\varPhi'$, simulating the actions in plan $\pi$, and measuring the difference between the simulated outcome of these actions and the observed trajectory $\tau$. 
The inconsistency score $C_{\varPhi'}$ serves two purposes. First, we keep track of the best repair generated so far, and return it when the search halts. Second, we consider a repair's inconsistency score when choosing which repair to pop from $OPEN$ in each iteration. This is embodied in the function $f(\varPhi', C_{\varPhi'})$ in line~\ref{alg:line:f} in Algorithm~\ref{alg:repair}. 
In our implementation, $f$ is a linear combination of the inconsistency score and the size of the repair, i.e., the number of MMOs it is composed of. The latter consideration biases the search towards simpler repairs. 

\begin{figure}
	\centering
	\includegraphics[width=0.9\columnwidth]{images/MMO_search_tree3.png}
	\caption{An example MMO search graph showing how a repair (a sequence of MMOs) is selected. The green node depicts a goal state in the MMO repair search, the minimal change to the model that causes the inconsistency score to fall below the set threshold.}
	\label{fig:mmo_search}
 \vspace{-3mm}
\end{figure}

Figure~\ref{fig:mmo_search} visualizes an example search tree of the MMO-based model repair algorithm where MMOs are treated as actions and the state is composed of changes to the default model (0 indicates no change to the given fluent). The inconsistency score is estimated for each generated repair, and the search terminates once a repair is found such that the updated domain $D'$ is consistent with the true transition function $T^*$. MMO repair is performed on a set of repairable fluents $\{x_1, x_2, ..., x_n\}$. Each MMO adjusts the value of a given fluent by a fixed amount $\Delta$ ($+\Delta$ or $-\Delta$), defined \emph{a priori} per fluent (denoted as delta in top left of Figure.~\ref{fig:mmo_search}). In this example scenario, the best repair $\varPhi_{best} = \{\varphi_3, \varphi_3, \varphi_3\}$ is a sequence of three MMOs (each adjusting $x_2$ by $+0.2$) such that repair $\varphi_{best}$ changes a single state variable $x_2 \in X$ by adding $0.6$ to its value.


\subsubsection{Focused Model Repair}

In many cases, allowing the repair to adjust multiple variables simultaneously can result in search space explosion. The branching factor of the general model repair algorithm is $2^n$. An impactful novelty usually requires significant change to the domain, high branching factor and vast search space might cause it to not be found within a reasonable time.

\begin{figure}
	\centering
	\includegraphics[width=0.9\columnwidth]{images/MMO_focused_search_tree3(1).png}
	\caption{Example MMO search graph for a focused model repair.}
	\label{fig:mmo_focused_search}
 \vspace{-4mm}
\end{figure}

To make repair feasible in complex domains, we introduce focused model repair, a restricted variant of the general algorithm. The two mechanisms differ only in how they expand new repair candidates. In the focused case, an additional constraint is imposed such that any repair candidate $\varPhi$ can only contain MMOs of the same type $\varPhi = \{\varphi_i, \varphi_i, ... , \varphi_i\}$ where $\varphi_i \in \{\varphi\}$. 
\roni{Need to better motivate the focused model repair. Why choosing only the same type of novelty is a good idea}
To implement focused repair, the aforementioned constraint is added after line 4 in Algorithm \ref{alg:repair}. The search graph of the focused model repair is shown in fig. \ref{fig:mmo_focused_search}.




==> problem.tex <==
\section{Problem Setup}
\label{sec:problem}

% Setting: the environment is a complex mixed discrete-continuous environment
We consider an agent acting in a complex discrete-continuous environment that is modeled as a transition system $E=\tuple{F, X, A, T}$ where 
$F$ is a set of discrete state variables;
$X$ is a set of numeric state variables; 
$A$ is a set of actions the agent may perform; 
and $T$ is a transition function that governs the dynamics of the environment. 
A \emph{state} of an environment is a complete assignment of values over all its state variables. We denote by $S$ the set of all possible states in the environment. 


% We consider a planning-based agent
To control the agent, we assume a planning-based agent that calls an automated planner to determine which actions to perform in order to achieve desired goals. 
Automated planners require a \emph{domain}, which is the planner's internal approximation of environment $E$, specified in a formal planning language. 


% We do PDDL+
To support rich environments with complex dynamics and discrete and numeric state variables, we assume a planner that uses domains specified in PDDL+~\cite{fox2006modelling}. 
A planning domain in PDDL+ defines how the state changes under various \emph{happenings} that include actions the agent may perform, exogenous events that may be triggered, 
and durative processes that may be active.
%\footnote{The effects of processes and events are implicitly applied via a time-passing action that the agent can apply alongside the actions defined in the PDDL+ domain.} Roni: I don't see this as relevant at athis stage
Each happening is represented as a pair of \emph{pre-conditions} and \emph{effects} expressed in terms of assignments and mathematical expressions. An example of a process from the CartPole++ domain is shown in Figure \ref{fig:process-cartpole}. 
A planning \emph{problem} $\mathcal{P}$ in a domain $\mathcal{D}$ is a pair $\mathcal{P}=\tuple{s_0,G}$ where $s_0\in S$ is the initial state., and $G \subseteq S$ is a set of possible goal states. A solution to a problem $\mathcal{P}$ is a plan $\pi = (a_0, a_1, ..., a_n)$ which reaches a goal state $s_G \in G$. Executing a plan $\pi$ in domain $\mathcal{D}$ yields a trajectory $\tau = (\tuple{s_0, a_0, s_1}, \tuple{s_1, a_1, s_2}, ... , \tuple{s_n, a_n, s_G})$, which comprises a sequence of tuples of the form $\tuple{s_i, a_i, s_{i+1}}$, representing that the agent performed action $a_i$ in state $s_i$, and reached state $s_{i+1}$.


\subsection{Novelties}
% Consistency and Novelties
In the nominal case, the agent's internal domain $\mathcal{D}$  models the environment $E$ in sufficient accuracy that a plan that achieves the goal according to $\mathcal{D}$ will also do so in $E$. When this relationship between $\mathcal{D}$ and $E$ occurs we say that they are \emph{consistent}, denoted by $\mathcal{D} \cong E$. 
In this paper, we study the case when a \emph{novelty} is introduced in the environment, after which, a new transition function $T^*$ begins governing environmental dynamics $E^*$. Consequently, $\mathcal{D}$ and $E$ become inconsistent. 
% What is the input the agent has
Specifically, we assume the planning-based agent interacts repeatedly with the environment for $N$ \emph{episodes}, similar to the standard Reinforcement Learning setting. 
Each episode begins in some initial state of the environment $s_0 \in S$. 
Then, the agent iteratively executes actions and observes their outcomes until a terminal state is reached. 
After an unknown number of episodes, a novelty is introduced, changing the environment. 
This change is expected to degrade the performance of the planning-based agent, since its internal domain is now inconsistent with the environment. 
The agent does not know when the novelty is introduced or how it has changed the environment. 
We refer to such a sequence of episodes as a \emph{trial}. 
Note that the trial does not end immediately after the novelty has been introduced, and the agent does not know a-priori the number of episodes in a trial. 
The main objectives of this work is to develop agents that can (1) detect in a trial the novelty has been introduced and (2) adapt to it so that it returns to perform effectively in the modified environment. We refer to the former as the \emph{novelty detection} problem and the latter as the \emph{novelty adaptation} problem. We say that an agent is \emph{novelty-aware} if it explicitly considers and addresses these two problems.

% Assumptions
In an open world, any number of novelties can present themselves at any timepoint. 
However, in this work we limited our scope by making the following assumptions: 
(1) novelty is introduced only between episodes; (2) at most one novelty is introduced per trial; (3) once a novelty is introduced, it persists for the remainder of the trial. We refer to this setup as the \emph{single persistent novelty setup}. 
We chose to make these assumptions to support iterative development of agents and allow clear experimental measurement. 
%, we impose some constraints.  We assume that, 

%At the beginning of the trial the environment operates with $T$, the canonical transition function. In some episode $k$ unknown to the agent, the transition function is updated to $T^*$ also unknown to the agent. An effective novelty response from the agent requires it to first detect \emph{when} the novelty was introduced and accommodate it by determining \emph{how} to update its model\footnote{The presented novelty trial setup is designed to clearly show adaptation to novelty. In practice, however, novelty can be introduced at any point and different novelties can be introduced in the trials. The adaptation mechanism can update the agent's internal model repeatedly for each introduced or removed novelty.}. REPETITION






% Our objective is to 
% modify $D$ such that it allows the agent to solve problems in $E^*$. We introduce a novelty reasoning method that takes as input, the agent's current internal domain $D$, plan $\pi$, and the observations trajectory $\tau$ created by the agent operating in $E^*$. The output is a \textit{modified internal domain $D^*$} that enables the agent to solve problems in $E^*$ i.e., $D^* \cong E^*$ 








% Our approach is built upon a model-based agent that calls a PDDL+ planner to determine a sequence of actions given a state and then, executes them in the environment. 
% %A planner represents the current state of the world as a set of grounded predicates $p(s_t) \subseteq P$ given the current observations (discrete variables $F$ and continuous variables $X$) in environmental state $s_t$. 
% To plan, domain $D$ is the agent's internal approximation of environment $E$, defining how the state changes under various \emph{happenings} that include actions, events that were triggered, and durative processes that are may be active\footnote{The effects of processes and events are implicitly applied via a time-passing action that the agent can apply alongside the actions defined in the PDDL+ domain.}. Each happening is represented as a pair of \emph{pre-conditions} and \emph{effects} expressed in terms of assignments and mathematical expressions. An example of a process from the CartPole++ domain is shown in Figure \ref{fig:process-cartpole}. A planning \emph{problem} $\mathcal{P}$ in the domain $D$ is a pair $\mathcal{P}=\tuple{s_0,G}$ where $s_0\in S$ is the initial state., and $G \subseteq S$ is a set of possible goal states. A solution to a problem $\mathcal{P}$ is a plan $\pi = (a_0, a_1, ..., a_n)$ which reaches a goal state $s_G \in G$. Executing a plan $\pi$ in domain $D$ yields a trajectory $\tau = (\tuple{s_0, a_0, s_1}, \tuple{s_1, a_1, s_2}, ... , \tuple{s_n, a_n, s_G})$, which comprises a sequence of tuples of the form $\tuple{s_i, a_i, s_{i+1}}$, representing that the agent performed action $a_i$ in state $s_i$, and reached state $s_{i+1}$.

% What is a novelty




% % Setting is RL-like. We have episodes
% Following the structure of reinforcement learning agents, an open world learning agent interacts repeatedly with the environment for $N$ \emph{episodes} in a \emph{trial}. Each episode begins in an initial state of the environment and executes actions until a terminal state is reached. Upon termination, the agent initializes and acts in the next episode in the trial. 





% We view novelty as a transformation of the environmental dynamics. In an open world, any number of novelties can present themselves at any timepoint. However, to support iterative development of agents and clear experimental measurement, we impose some constraints. We assume that, (1) novelty is introduced only between episodes; (2) at most one novelty is introduced; (3) once a novelty is introduced, it persists for the remainder of the trial. We refer to this setup as the \emph{single persistent novelty setup}. At the beginning of the trial the environment operates with $T$, the canonical transition function. In some episode $k$ unknown to the agent, the transition function is updated to $T^*$ also unknown to the agent. An effective novelty response from the agent requires it to first detect \emph{when} the novelty was introduced and accommodate it by determining \emph{how} to update its model.

% \textcolor{red}{Shouldn't we add some background, similar to the recent IJCAI submission? $\sim$ Sachin}

% An environment in our context can be considered as a transition system $E=\tuple{F, X, A, T, G}$ where 
% $F$ is a set of discrete variables;
% $X$ is a set of numeric state variables; 
% a state $s \in S$ is a complete assignment of values to the state variables $S = F \cup X$; % Johan: is S not part of E?  What is it part of.
% $A$ is a set of agent actions and includes a null representing no deliberate action by the agent; 
% $G \subseteq S$ is a finite set of goal states;
% % goal $G \in \mathcal{G}$ is a possibly partial assignment of values of the state variables $F\cup X$ and is a terminal state in the environment;
% model $T: S \times A \rightarrow S$ is a transition function that governs the dynamics of the environment (i.e., $T(s, a) \rightarrow s'$).
% % $R$ is a reward function $R: R(s) \rightarrow \mathbb{R}$, where $R(s)$ returns the reward of reaching state $s$. 



% % Our approach is built upon a model-based agent that calls a PDDL+ planner to determine a sequence of actions given a state and then, executes them in the environment. 
% % %A planner represents the current state of the world as a set of grounded predicates $p(s_t) \subseteq P$ given the current observations (discrete variables $F$ and continuous variables $X$) in environmental state $s_t$. 
% % To plan, domain $D$ is the agent's internal approximation of environment $E$, defining how the state changes under various \emph{happenings} that include actions, events that were triggered, and durative processes that are may be active\footnote{The effects of processes and events are implicitly applied via a time-passing action that the agent can apply alongside the actions defined in the PDDL+ domain.}. Each happening is represented as a pair of \emph{pre-conditions} and \emph{effects} expressed in terms of assignments and mathematical expressions. An example of a process from the CartPole++ domain is shown in Figure \ref{fig:process-cartpole}. A planning \emph{problem} $\mathcal{P}$ in the domain $D$ is a pair $\mathcal{P}=\tuple{s_0,G}$ where $s_0\in S$ is the initial state., and $G \subseteq S$ is a set of possible goal states. A solution to a problem $\mathcal{P}$ is a plan $\pi = (a_0, a_1, ..., a_n)$ which reaches a goal state $s_G \in G$. Executing a plan $\pi$ in domain $D$ yields a trajectory $\tau = (\tuple{s_0, a_0, s_1}, \tuple{s_1, a_1, s_2}, ... , \tuple{s_n, a_n, s_G})$, which comprises a sequence of tuples of the form $\tuple{s_i, a_i, s_{i+1}}$, representing that the agent performed action $a_i$ in state $s_i$, and reached state $s_{i+1}$.

% % In the nominal case, the agent's internal domain $D$ closely models the environment $E$ and are called \emph{consistent}; 
% % We denote this consistency by $D \cong E$. In this paper, we study the case when a novelty is introduced in the environment, after which, a new transition function $T^*$ begins governing environmental dynamics $E^*$. Consequently, $D \ncong E$, they become inconsistent. Our objective is to modify $D$ such that it allows the agent to solve problems in $E^*$. We introduce a novelty reasoning method that takes as input, the agent's current internal domain $D$, plan $\pi$, and the observations trajectory $\tau$ created by the agent operating in $E^*$. The output is a \textit{modified internal domain $D^*$} that enables the agent to solve problems in $E^*$ i.e., $D^* \cong E^*$ 


\subsection{Case Studies}
Throughout this paper, we consider three different domains as case studies for the agent design we propose: Science Birds, Cartpole++, and Polycraft. We provide a brief description of these domains and instances of the single persistent novelty setup in them. 


\subsubsection{Science Birds}
Science Birds (SB) is a version of the popular video game Angry Birds, which has garnered widespread recognition over a substantial number of years. The objective in SB involves eliminating all green pigs in a level while maximizing destruction to the surrounding structures. The player is equipped with a collection of birds, which may vary, to be launched from a slingshot. The pigs are typically concealed within complex structures, requiring the player to identify and eliminate the weak points of the structures, such as supports or dynamite. The development of Science Birds utilized the Box2D open-source physics library, ensuring that all objects within the game's environment comply with the principles of Newtonian physics in a two-dimensional plane.
Table ~\ref{tab:sb_novelties} lists examples of novelties in SB, as published by Renz et al.~\cite{renz2019ai}. 
 The novelties of Science Birds are divided into three phases based on their order of release date. Each phase of novelties contains different levels and types corresponding to the difficulties posed by the induced novelties in the game. 


 \subsubsection{Cartpole++}
Cartpole++ is a physics-based discrete-continuous domain. The CartPole++ environment (seen in figure \ref{fig:cartpole}) is a higher-dimensional version of the standard Reinforcement Learning benchmark problem Cartpole. The agent can push the cart in any of the cardinal directions and the objective is to leave the pole upward for 200 steps. 
An example of a novelty in this domain can be that the mass of the cart suddenly increases or the length of the pole grows. 


\subsubsection{Polycarft}
\begin{figure}
\centering
\includegraphics[width=\textwidth]{images/polycraft_environment.png}
\caption{Top- and first-person view of the simulated environment for polycraft. Steve interacts with environment by sending sequence of commands such as ``SENSE\_ALL'' or ``BREAK BLOCK'' for cutting trees of mining ores in the environment.}
\label{fig:polycraft_environment}
\end{figure}

Polycarft is version of the popular video game MineCraft\footnote{\url{https://www.minecraft.net/}}. 
In Polycraft, we control an agent (Steve) that interacts with the environment, e.g., gathering resources such as logs by cutting trees, mining ores of diamond, interact with other entities such as traders to trade for several other resources, and follow a recipe to craft a new item. The Polycraft game has different tasks for the agent, but we focused on the ``Build a Pogostick'' task, where
the agent is tasked to craft a pogo stick. Crafting a pogostick requires sequential decision-making including both short and long-term planning. For example, the agent has to decide to collect resources needed to craft intermediate products, such as, a tree tap, and then use it to collect rubber from a specific kind of a tree in the environment. Figure \ref{fig:polycraft_environment} shows the top- and first-person view of the environment that consists of 30x30 grass field, and is connected to two smaller rooms. 
Examples of novelties in this domain are changing the quantity of raw material that can be extracted from their ores, or wind in the environment that changes the location of the agent while moving in the environment. 

\roni{I do not think we need more details about these domains here. The rest of the details should be pushed to the experimental setup part later in the paper.}

%A trial in polycraft environment consists of 50-100 episodes, and the novelty is introduced roughly after $20\%$ of the episodes have been completed. The agent should report the novelty after it has been introduced and update it's own transition function to incorporate the effects of novelty.



% Steve has the ability to interact with the environment by sending commands to the simulator. For example, steve can sense the environment by sending ``SENSE\_ALL'' command to the simulator and the simulator responds with the entities in the environment, their location, Steve's inventory, etc. Each action executed in the simulator has some cost attached to it (in the order of 1000 points), and Steve is rewarded with 256,000 points for a constructing a pogostick. The final score (reward - cost of executing all the actions) is presented after completion of the episode.

%Although, constructing a pogostick has it's own challenges, diverging $T^*$ due to novelty provides a completely new challenge for the agent. Novelties can support/hinder the construction of the pogostick, such as, by changing the quantity of raw material from their ores, or wind in the environment that changes the location of the agent while moving in the environment. A trial in polycraft environment consists of 50-100 episodes, and the novelty is introduced roughly after $20\%$ of the episodes have been completed. The agent should report the novelty after it has been introduced and update it's own transition function to incorporate the effects of novelty.




% , with more actions and state variables. The planning agent relies solely on PDDL+ model of the CartPole++ environment to solve the non-novel instances. For each episode, the agent generates a problem file from the initial environment observation (i.e., initial positions and velocities of the cart and pole) and default assumptions about the environment (i.e., gravity, masses of cart and pole, etc.). The expressiveness of PDDL+ enabled us to holistically encode the CartPole++ system dynamics as a planning domain (without using any external functions/solvers). Despite inherent complexity, efficient modeling allowed the use of off-the-shelf PDDL+ planners to solve the resulting problems. The planners were required to handle non-linear dynamics, large numbers of active happenings, and long temporal horizons.
% Depending on the initial positions, our planner can solve full 200-step CartPole PDDL+ problems in under $1.0$ second using GBFS algorithm with a domain specific heuristic prioritizing ``safe" states (pole close to the vertical). To account for the inherent noise between the planner and the execution environment, every 10 steps the agent re-plans for the remainder of the episode. 

 
%  A detailed description of each novelty is presented in Table ~\ref{tab:sb_novelties}.
% Examples of noveltis in SB include 



% In this context, the Science Birds game used is a modified-dimensional version of the standard Science Birds benchmark, incorporating various novelties. The novelties of Science Birds are divided into three phases based on their order of release date. Each phase of novelties contains different levels and types corresponding to the difficulties posed by the induced novelties in the game. A detailed description of each novelty is presented in Table ~\ref{tab:sb_novelties}.



